Dive into Layers: Neural Network Capacity Bounding using Algebraic Geometry

The empirical results suggest that the learnability of a neural network is directly related to its size. To mathematically prove this, we borrow a tool in topological algebra: Betti numbers to measure the topological geometric complexity of input data and the neural network. By characterizing the expressive capacity of a neural network with its topological complexity, we conduct a thorough analysis and show that the network's expressive capacity is limited by the scale of its layers. Further, we derive the upper bounds of the Betti numbers on each layer within the network. As a result, the problem of architecture selection of a neural network is transformed to determining the scale of the network that can represent the input data complexity. With the presented results, the architecture selection of a fully connected network boils down to choosing a suitable size of the network such that it equips the Betti numbers that are not smaller than the Betti numbers of the input data. We perform the experiments on a real-world dataset MNIST and the results verify our analysis and conclusion. The code is publicly available.

==> content/proof_main.tex <==
\subsection{Proof of Lemma~\ref{lemma:polynomial}}
\input{content/proofs/Lemma_polynomial}


==> content/proofs/Def_double_complex.tex <==
	\begin{definition}[Double complex]
		A double complex  is a bi-graded Abelian groups 
		$$E^{\bullet, \bullet} = \bigoplus_{p, q} E^{p,q} $$
		equipped with the two homomorphisms
			$$ d_h : E^{\bullet, \bullet} \rightarrow E^{\bullet,\bullet+1} , \quad d_v :E^{\bullet, \bullet} \rightarrow E^{\bullet+1 ,\bullet}$$
		satisfying the conditions:
			$$d_h^2 =  d_v^2 = d_vd_h + d_hd_v=0$$
	\end{definition} 
	the above equations give the $D^2 = 0 $ if we define $D = d_h +d_v$ and without generality, let $$E^{p,q}=0, p <0 \text{ or } q <0$$ and a double complex can induce a single complex
	\begin{definition}[total complex]
		The total complex associated to a double complex $\{E^{\bullet,\bullet}, d_h, d_v\}$ is the complex $\{T^{\bullet}(E), D\}$ where 
		$$T^n(E) := \bigoplus_{p+q=n}E^{p,q}$$
	\end{definition}
	
	With the double complex associated its total complex, A complex of Abelian groups $\{C^{\bullet}, d\}$ can be approximated under the following commute diagram:
	
	$$\xymatrix{
		               & \vdots                           & \vdots                          & \vdots                          &  \\   
		0 \ar[r]^{d_h} & E^{0,1} \ar[r]^{d_h}\ar[u]^{d_v} & E^{1,1}\ar[r]^{d_h}\ar[u]^{d_v} & E^{2,1}\ar[r]^{d_h}\ar[u]^{d_v} &\cdots \\
		0 \ar[r]^{d_h} & E^{0,0} \ar[r]^{d_h}\ar[u]^{d_v} & E^{1,0}\ar[r]^{d_h}\ar[u]^{d_v} & E^{2,0}\ar[r]^{d_h}\ar[u]^{d_v} &\cdots \\
		0 \ar[r]^{d}   & C^{0}   \ar[r]^{d}  \ar[u]^{\phi}& C^{1}  \ar[r]^{d}  \ar[u]^{\phi}& C^{2}  \ar[r]^{d}  \ar[u]^{\phi}&\cdots \\
		               & 0 		             \ar[u]       & 0 		             \ar[u]     & 0 		             \ar[u]   &
	}
	$$
	In particular, if we have the condition:
	\begin{definition}[resolution]
		A resolution of the complex $\{C^{\bullet},d\}$ by a double complex$\{E^{\bullet, \bullet}, d_h, d_v\}$ is a homomorphism $\phi: \{C^{\bullet}, d\}\rightarrow \{E^{\bullet, \bullet}, d_h, d_v\}$ such that the columns in the above diagram are exact. In another word, we have the long exact sequence:
		$$0\hookrightarrow C^n \stackrel{\phi}{\longrightarrow} E^{n,0} \stackrel{d_v}{\longrightarrow} E^{n,1} \stackrel{d_v}{\longrightarrow} \cdots$$
	\end{definition}

==> content/proofs/Def_exact_sequence.tex <==
	\begin{definition}[exact sequence]
		A sequence 
		$$\cdots \rightarrow G_0  \stackrel{f_0}{\longrightarrow} G_1 \stackrel{f_1}{\longrightarrow} G_2 \stackrel{f_2}{\longrightarrow}  \cdots$$
		of groups and group homomorphisms is called exact if the image of  each homomorphism  is equal to the kernel of the next:
		$$Img(f_k) = Ker(f_{k+1})$$
		the sequence of groups and homomorphism may be either finite or infinite.
	\end{definition}

==> figure/betti_bounding.tex <==
\begin{table}[!ht]
\begin{minipage}{0.5\linewidth}

    \centering
    \begin{tabular}{m{0.7cm}m{0.7cm}|m{0.7cm}m{0.7cm}}
    % \hline
    % \multicolumn{6}{c}{Polynomial case} \\ 
    \hline
    \multicolumn{2}{c}{node number = 2} & \multicolumn{2}{c}{node number = 3} \\
    \hline
      layer &  bound   & layer &  bound   \\
    
       1  &  36        & 1 & 196  \\ 
     
       2 & 6           & 2 & 18  \\
  
       3 & 1           & 3 & 1  \\
       \hline
    \end{tabular}
    \caption{polynomial}
    \label{tab:poly}

\end{minipage}%
\begin{minipage}{0.5\linewidth}
    \centering
    \begin{tabular}{m{0.7cm}m{0.7cm}|m{0.7cm}m{0.7cm}}
    % \hline
    % \multicolumn{6}{c}{ReLU case} \\ 
    \hline
    \multicolumn{2}{c}{node number = 2} & \multicolumn{2}{c}{node number = 3} \\
    \hline
      layer & bound  & layer & bound    \\
    
       1  & 728      & 1 & 19682  \\ 
     
       2 & 80        & 2 & 728   \\
  
       3 & 8         & 3 & 26  \\
       \hline
    \end{tabular}
    \caption{ReLU }
    \label{tab:relu}
\end{minipage}
\end{table}
